Execution at RISC: Stealth JOP Attacks on RISC-V Applications

RISC-V is a recently developed open instruction set architecture gaining a lot of attention. To achieve a lasting security on these systems and design efficient countermeasures, a better understanding of vulnerabilities to novel and potential future attacks is mandatory. This paper demonstrates that RISC-V is sensible to Jump-Oriented Programming, a class of complex code-reuse attacks. We provide an analysis of new dispatcher gadgets we discovered, and show how they can be used together in order to build a stealth attack, bypassing existing protections. A proof-of-concept attack is implemented on an embedded web server compiled for RISC-V, in which we introduced a vulnerability, allowing an attacker to remotely read an arbitrary file from the host machine.

==> Makefile <==
ART_SRCS = article.tex \
		   intro.tex \
		   background-cra.tex \
		   riscv_jop.tex \
		   experiment.tex \
		   conclusion.tex \
		   related.tex

BIB_SRCS=bibliography.bib
EXTRA_SRCS=llncs.cls splncs04.bst
SRCS=$(ART_SRCS) $(BIB_SRCS) $(EXTRA_SRCS) Makefile

all: wasp-2023.pdf

wasp-2023.pdf: $(SRCS)
	latexmk -emulate-aux-dir -aux-directory=auxdir -output-directory=outdir --output-format=pdf $<
	cp outdir/article.pdf $@

clean:
	latexmk -emulate-aux-dir -aux-directory=auxdir -output-directory=outdir --output-format=pdf -C $<

clean-all: clean
	rm -f wasp-2023.pdf
	rm -rf auxdir
	rm -rf outdir


==> attack_surface.tex <==
\section{RISC-V attack surface}\label{sec:attack-surface}

JOB attacks rely on the ISA and ABI of the target, and as such they
represent the attack surface of the target.
In this section we present the RISC-V ISA and ABI elements and properties of
interest for the realisation of JOB attacks.

Note that the ABI is purely a convention, i.e. while an application on a RISC-V
processor must follow the RISC-V ISA specificiations, it is not mandatory to
follow any particular ABI.
In this article, we made the hypothesis that the target application binary and
all related software artifacts were generated (e.g. compiled) following the
convention described in Chapter 18 of the RISC-V specification\cite{rvspecs}.

\subsection{ISA: Instruction Set Definition}
\label{ref:riscv-isa}

The RISC-V ISA defines multiple extensions to the base instruction set.
Amongst these extensions, only the Base Integer ISA (RV32I) is mandatory in all
RISC-V implementations. Depending on supported extensions, new registers
will be available (e.g. floating registers). A 16-bits compressed version
of Base Integer ISA is also available. Available registers in the target
architecture will strongly impact its attack surface relatively to JOP
attacks, as more gadgets will be eligible when more registers are present.

In our experiment, we had the most possible conservative approach by only
considering the Base RISC-V ISA and the Base Integer ISA, thus exploiting a
minimal attack surface. Any added extension will increase the likelihood of
finding gadgets within the target application.

\subsection{ISA: Instructions Alignment}

The number of gadgets available is increased if the instructions are not
aligned, since in the latter case, instructions may be loaded after their
intended beginning, and thus interpreted with unintended opcodes and
arguments~\cite{Jaloyan20}. Contrary to CISC architectures such as
x86, RISC-V being a RISC architecture, RISC-V instructions have a fixed size.
However, an extension providing compressed instructions (RV32C and RV64C)
is defined in the standard, although not mandatory. RISC-V implementations
supporting this extension may be target to instruction offset shifting
attacks, where the attacker jumps after the begining of an instruction and
thus execute unintended instructions.

\subsection{ISA: Instructions of Interest}

Designing a JOP attack relies on chaining functional gadgets. This chaining is
performed by using control transfer instructions exploiting registers as jump
target designator. In the RISC-V Base Integer ISA, there is only one instruction
allowing such operation: the Jump-And-Link-Register instruction (JALR), as
illustrated in Figure~\ref{fig:cva6jalr}.

\begin{figure}
\includegraphics[scale=0.6]{figs/cva6_jalr.png}
\caption{RISC-V Jump-And-Link-Register instruction}\label{fig:cva6jalr}
\end{figure}

JALR computes the target address for the control transfer by adding a 12-bits
signed immediate to the rs1 register, then setting the least-significant bit
of the result to zero, allowing to reach +/- 2 ko from the source address.
Reachable addresses can be further extended by using the Add Upper Immediate
to PC (AUIPC) instruction, which add 20 bits to the memory, effectively making
all the physical memory addressable with the immediate. In the case of a JOP
attacks, exact addresses of the gadgets are stored into the dispatch table
and loaded directly into \emph{rs1} (one register argument), so immediate is
set to zero and thus no AUIPC instruction is needed by the attacker.

\subsection{ABI: Registers of Interest}

JOP attacks exploit instructions allowing jumping to an address stored within a
register. The Base Integer ISA from RISC-V defines 32 generic registers usable in
user mode:
\begin{itemize}
\item a global pointer addressing different symbols (functions, global variables)
  within the application;
\item a return register containing the return
  address of the last caller function;
\item a stack pointer;
\item a thread pointer;
\item 8 argument registers, used to pass arguments to functions;
\item 6 temporary registers, used to store intermediary results;
\item 12 save registers, used by compiler to otimize access to non-volatile values
  accessed from different functions.
\end{itemize}

Table~\ref{tab:rvabi} shows the registers mnemonics and usage purpose as defined
by the RISC-V specification ABI.
As shown in the table, the ABI states that return, argument and temporary
registers are the only registers saved by caller functions.

% \begin{table}
% \includegraphics[scale=0.75]{figs/riscv-abi.png}
%   \caption{RISC-V registers usage as describe by ABI}\label{tab:rvabi}
% \end{table}

% \begin{table}[h]
%   \scriptsize
%   \begin{center}
%     \begin{tabular}{|p{4em}|p{4em}|p{9.5em}|p{3em}|}
%       \hline
%       Register & ABI Name & Description & Saver \\
%       \hline
%       x0 & zero & Hard-wired zero & --- \\
%       x1 & ra & Return address & Caller \\
%       x2 & sp & Stack pointer & Callee \\
%       x3 & gp & Global pointer & --- \\
%       x4 & tp & Thread pointer & --- \\
%       x5 & t0 & Temporary/alternate link register & Caller \\
%       x6-7 & t1-2 & Temporaries & Caller \\
%       x8 & s0/fp & Saved register/frame pointer & Callee \\
%       x9 & s1 & Saved register & Callee \\
%       x10-11 & a0-1 & Function arguments/return value & Caller \\
%       x12-17 & a2-7 & Function arguments & Caller \\
%       x18-27 & s2-11 & Saved registers & Callee \\
%       x28-31 & t3-6 & Temporaries & Caller \\
%       \hline
%     \end{tabular}
%   \end{center}
%   \caption{RISC-V registers usage as describe by ABI}\label{tab:rvabi}
% \end{table}

\begin{table}[h]
  \scriptsize
  \begin{center}
    \begin{tabular}{|p{4em}|p{3em}|p{9em}|p{3em}|}
      \hline
      Register & ABI Name & Description & Saver \\
      \hline
      x0 & zero & Hard-wired zero & --- \\
      x1 & ra & Return address & Caller \\
      x2 & sp & Stack pointer & Callee \\
      x3 & gp & Global pointer & --- \\
      x4 & tp & Thread pointer & --- \\
      x5 & t0 & Temporary / alternate link register & Caller \\
      x6-7 & t1-2 & Temporaries & Caller \\
      \hline
    \end{tabular}
    \begin{tabular}{|p{4em}|p{3em}|p{9em}|p{3em}|}
      \hline
      Register & ABI Name & Description & Saver \\
      \hline
      x8 & s0/fp & Saved register / frame pointer & Callee \\
      x9 & s1 & Saved register & Callee \\
      x10-11 & a0-1 & Function arguments / return value & Caller \\
      x12-17 & a2-7 & Function arguments & Caller \\
      x18-27 & s2-11 & Saved registers & Callee \\
      x28-31 & t3-6 & Temporaries & Caller \\
      \hline
    \end{tabular}
  \end{center}
  \caption{RISC-V registers usage as describe by ABI}\label{tab:rvabi}
\end{table}

\subsection{ABI: Convention on Function Calls}

Convention on RISC-V function calls favors passing arguments by registers
when possible. Eight integer registers are saved for this purpose in the RV32I.
When no register is available, arguments are stored in the stack.

As mentioned in Section~\ref{introcra}, CRA in general and JOP in particular consist in
using existing functions and system calls within the target application.
Since the behaviour of these functions and system calls is controlled by their
parameters, those will be the favorite targets for an attacker. Two information
in particular are interesting regarding argument passing: (1) assignment of
registers and (2) layout of parameters' values within these registers. In the
next subsections, we use the XLEN term to describe the registers size in bits (32 or 64
according to the RISC-V architecture).

\subsection{ABI: Argument Registers Allocation}

Arguments with a size equal or less than XLEN are assigned to registers
according to their position within the function's signature, e.g. first
argument is assigned to first argument register (a0), second argument is
assigned to second argument register (a1) and so on. Arguments with a size
greater than 2*XLEN are passed by reference (so they occupy a single register).
Finally, arguments with a size greater than XLEN and less or equals to 2*XLEN use
a pair of registers. Hence in the case of manipulation of data belonging to the
latter group (such as \textit{long long} in a RV32I), more arguments
registers than actual arguments will be used. This makes the application more
likely to use upper argument registers. Since the number of argument registers
used in the application is a strong limitation in the attacker ability to find
gadgets due to our approach (see~\ref{ref:craft_jop}), this pattern increases
its vulnerability against JOP.

\subsection{ABI: System Calls}
\label{ref:riscv-syscalls}

In RISC-V system calls are performed through the ecall instruction. Each
system function has an integer identifier allowing identification during the
call. This identifier must be set into the last argument register (a7) before
call execution. If any arguments are necessary to the system call, they must be
passed through the other argument registers (a0-a7).

While it is possible to manipulate a7 to change any syscall to the desired one,
we found that their was not many occurrences of manipulation of a7 outside of
setting of syscalls and without of adversary side-effects on lower argument
registers. Hence, we rather identified within the application the system call
of interest, which was easy in our case, since we target the commonly used
\emph{write} syscall.


==> craft_jop.tex <==
\section{Crafting a JOP Chain for RISC-V applications}
\label{ref:craft_jop}

As mentioned in Section~\ref{ref:riscv-isa}, we adopted a conservative approach regarding
our selection of registers of interest. We used the same approach regarding their
exploitation: we defined a subset of register of interest to be \emph{reserved registers},
that are used by the attack to store addresses necessary to the continuity of the
attack. These registers are:
\begin{itemize}
  \item \emph{a5}, the gadget dispatcher address (which can consists in one or two
    addresses, depending on the kind if gadget dispatcher);
  \item \emph{a4}, the current entry in the dispatch table.
\end{itemize}

We did not consider in our experiment the possibility to save and restore these
registers' values, so any writing on the registers by any gadget after the gadget
initialization will interrupt the attack. To find a way to save/restore these
registers (either through memory or through direct register copy) would considerably
ease the finding of gadgets and the crafting of the JOP chain.

\subsection{JALR Instruction}

The Jump-And-Link-Register instruction may be generated by the compiler when the
code tries executing a function pointer. The specific case of JALR performed
on a parameter happens when said function pointer was passed to the parent
function through arguments -- in that case, JALR will jump to the address
contained in the related argument. Hence manipulating this argument allows
modifying the execution flow.

For example, a generic comparison function would take as arguments 2 structures
to be compared, and a pointer on a comparison function. The two structures will
occupy registers a0 and a1 (supposing they fit in), and the comparison function
address will be stored in register a2. When calling the comparison function, the
generic comparison function will use a JALR (depending on compiler options) and
branch to register a2, as illustrated in Figure~\ref{fig:jalr}. The generic function
is a good candidate for chaining JOP gadgets, as it allows taking control of
execution flow with the assumption that the arguments are already controlled by
the attacker.

\begin{figure}
\includegraphics[scale=0.5]{figs/jalr_pattern}
\caption{Pattern generating vulnerable JALR}\label{fig:jalr}
\end{figure}

\subsection{Dispatcher Gadget}\label{subsec:dispatcher-gadget}

The dispatcher gadget is an essential part of any JOP attack. Its behaviour is
similar to an instruction pointer, as it allows (1) loading an address in the
dispatch table, (2) jumping to said address and (3) moving to the next gadget
table entry. The dispatch table is typically injected in the application through
through the buffer that was used to initiate the attack. The execution
order of gadgets is generally sequential, but it may be more complex, according
to available dispatcher gadget candidates in the application. In any case, it is
defined by the dispatch table layout which is crafted by the attacker during the
weaponization phase of the attack (as defined in Lockeed Martin cyber kill 
chain\footnote{https://www.lockheedmartin.com/en-us/capabilities/cyber/cyber-kill-chain.html}).

While its expected behaviour is simple, to find an ideal dispatcher gadget is a
difficult task. In the case of a RISC-V application, the attacker must find the
following pattern:
\begin{itemize}
  \item one instruction to increment a1 (supposing the dispatch table was
    stored there);
  \item one instruction loading a2 from a1 (were a2 will contain the next
    address to be jumped to);
  \item one instruction to perform an indirect jump (JALR) to the address stored
    in a2.
\end{itemize}
While other instructions may be interlacing with the instructions above, they must
not tamper with either a1 or a2 (neither any registers used in further
operations, such as the one containing the address of the gadget dispatcher
itself). While this issue may be solved by using other registers than argument
registers, another solution to address this issue is to use a 2-stage gadget
dispatcher, as proposed by~\cite{joprocket21}. In that case, the
first ``stage'' of the dispatcher gadget is effectively a gadget allowing to parse
the dispatch table (generally by incrementing a pointer), and then branches on the
second stage, which in turn performs a load on the dispatch table current position,
and then branches on this value using the JALR instruction. Figure~\ref{fig:2stages}
illustrates a 2-stage dispatcher gadget on RISC-V.

\begin{figure}
\includegraphics[scale=0.7]{figs/2stage_gadget_dispatcher}
\caption{2-stage gadget dispatcher}\label{fig:2stages}
\end{figure}

\subsection{Functional Gadgets}\label{subsec:func-gadgets}

The dispatcher gadget is only useful if it can address the functional gadgets
needed to perform the attack. There are different families of functional gadgets,
as described for ROP attacks by~\cite{bletsch11}:
\begin{itemize}
\item arithmetic and logic gadgets
\item memory access gadgets
\item function call gadgets
\item system call gadgets
\item branching gadgets
\end{itemize}
Even in ROP attacks, one or more gadgets of each of these families need
(e.g. memory access will require a loader and a saver gadget) to be present in
order to achieve Turing-completeness~\cite{Cheng11}.
In the case of JOP attacks were more than one register may be exploited to chain
the gadgets, the number of gadgets needed may increase even further.

Reaching Turing-completeness however, although intellectually satisfying, is
often not needed to perform an actual attack -- hence the question whether 
there is enough functional gadgets available in an application to perform an 
attack is hard to answer, particularly since the attacker may adapt the attack 
to available gadgets. In our experiment we did not aim for Turing-completeness, 
so we did not need all the gadgets types listed above. We needed, and were 
able to find (or rather to generate in our vulnerable application) (1) 
arithmetic gadgets, (2) memory access gagdets and (3) system call gadgets. 

In addition to these functional gagdets, we also needed a initializing gagdet, 
which is a one-shot functional gadget used to configure the registers containing 
the dispatcher gadget and the dispatch table addresses. While it is actually a 
memory access gadget in literature, its specific role makes it unique, as it will 
be the only gadget allowed to write in the reserved registers.

\subsubsection{Arithmetic and logic gadgets}

As suggested by their name, arithmetic and logic gadgets are used to perform
arithmetic and logic operations on registers' values. During our experiment, we
focused on argument registers, thus one needs to find a gadget performing the
needed operations on the current function parameters. An example of an AND operation
executed on arguments of a function is provided in Figure~\ref{fig:andgadget}.

\begin{figure}
\includegraphics[scale=0.7]{figs/and_gadget}
\caption{AND gadget}\label{fig:andgadget}
\end{figure}

\subsubsection{Memory access gadgets}\label{subsubsec:mem-access-regs}

Memory access gadgets are the most important gadget in any attack scenario -- second only to
system call gadgets. They allow reading and writing values from/into memory, and are always
necessary to parametrize said system calls, but also more generally to access
sensitive data. One simple example is to write in memory the name of a sensitive
file in file system (e.g. /etc/shadow in a Linux context) and then calling the
syscall \emph{open}, allowing tampering of said file (providing the target
application has root privilege) and thus allowing the attacker to modify users'
passwords. 

Memory access gadgets can be found, amongst other places, in functions manipulating
structures. As these structures' size is typically greater than XLEN*2, they are
passed by reference, and then a memory read will be performed. Conversely,
modification on the values of the structure parameters will be performed through memory
writings.

The location of writing and reading depends on the structure address, passed
through a register. Manipulating this register allows arbitrary reading or writing
within the memory (e.g. the dispatch table).

\subsubsection{System call gadgets}

As mentioned in Section~\ref{ref:riscv-syscalls}, system calls following the
RISC-V ABI use argument register a7 to pass the ecall identifier. Since argument
registers are assigned lower index first, finding functions manipulating a7 out of
system libraries is possible, yet very likely to lead to side effects on lower 
argument registers. In our research, we did not found gagdets manipulating a7 
without overwriting one of the reserved registers. Hence performing system calls 
practically means branching into related primitives in system libraries while 
ensuring a configuration of registers that will trigger the kernel action expected 
by the attacker.

Practically, that means we exploit entries into the Procedure Linkage Table (PLT).
This table and related functions are generated by the Linker during the linking
phase and points towards used functions in the libraries linked to the
application. From these addresses, we have an entrypoint to functions of interest
(e.g. open in libc), and then we can jump up to a fixed offset of the function 
with the instruction of interest (in our case, the instruction setting a7), and 
then executing the syscall.

